Learning to Learn in Simulation

Deep learning often requires the manual collection and annotation of a training set. On robotic platforms, can we partially automate this task by training the robot to be curious, i.e., to seek out beneficial training information in the environment? In this work, we address the problem of curiosity as it relates to online, real-time, human-in-the-loop training of an object detection algorithm onboard a drone, where motion is constrained to two dimensions. We use a 3D simulation environment and deep reinforcement learning to train a curiosity agent to, in turn, train the object detection model. This agent could have one of two conflicting objectives: train as quickly as possible, or train with minimal human input. We outline a reward function that allows the curiosity agent to learn either of these objectives, while taking into account some of the physical characteristics of the drone platform on which it is meant to run. In addition, We show that we can weigh the importance of achieving these objectives by adjusting a parameter in the reward function.

==> experiments_field.tex <==
We validated our curiosity agent on real-world imagery. In doing so, we both test our curiosity agent's generalizability, and its strategy's suitability to real-world targets. Note that the curiosity agent here is identical to the one in Section~\ref{sec:experiments_simulation}, and \textit{was trained purely on simulated scenes}.

We recorded several scenes (Figure~\ref{fig:screenshots}) with similar parameters to the simulated ones described in Section~\ref{sec:problem}. We again set $\Delta \alpha = 12\degree$, and $\theta = 30\degree$ to match the viewpoint of our training scenes. For the car and helicopter scenes, $d = 60$m. We reduced $d$ to 20m for the person scene, as the target was only several pixels in width at 60 meters. 

\begin{figure} \centering
    \includegraphics[width=0.9\linewidth]{field_orbits}
    \caption{Sample views from three field scenarios with three different targets (car, person, helicopter wreckage). All three scenarios exhibit views with varying degrees of obstruction and background clutter, with the first two explicitly created to have total obstruction and objects of the same class within the views. The helicopter wreckage represents a scene where the shape of the object varies at different view angles.}
    \label{fig:screenshots}
\end{figure}

By flying the exploration space and capturing each view using a drone, we were able to re-create arbitrary episodes with different strategies. We set the time budget $T=240$---at 2.5 seconds per time-step, this approximates the 10 minute flight time of our Jetson TX2-equipped drone.  To remove the effect of start position, we evaluated each of the 3 scenes in 5 separate episodes, starting at evenly spaced views around the orbit. We measured the resulting trainee performance and user interactions, and averaged them over the 15 total episodes. Figure~\ref{fig:sim_avg_itb_field} shows the user interaction effectiveness vs. time-step for each of the strategies, and Table~\ref{tab:simulation_results_field} quantifies these results.

% \begin{figure} \centering
%     \includegraphics[width=\linewidth]{sim_timeseries}
%     \caption{(top) Plot of AP vs. time-step for 3 real-world scenes. We see that all strategies perform similarly in AP, but vary vastly in terms of number of user interactions required to get there.}
%     \label{fig:sim_timeseries_field}
% \end{figure}

\begin{figure} \centering
    \includegraphics[width=1\linewidth]{field_avg_itb}
    \caption{}
    \label{fig:sim_avg_itb_field}
\end{figure}

We note that \textbf{orbit} dominates when it comes to $P$, more so than in the simulated cases. This is especially true for the helicopter scene, where the target is vastly different in appearance depending on view, and a brute-force annotation strategy is optimal. We believe decreasing $w_p$ in the reward function would help close this gap for such scenes, at the cost of more user interactions. Nevertheless, we observe that when it comes to $\overline{ITB}$, the curiosity agent again dominates the baseline strategies, by 2.27 times the next best strategy, \textbf{jump 10}. Versus \textbf{random}, the curiosity agent produces more than 8 times $\overline{ITB}$ per user interaction. 

\begin{table}[h]
\resizebox{\linewidth}{!}{%
  \begin{tabular}{ c | c | c | c | c }
    \hline
    \textbf{Strategy} & $P_{240}$& $\sum_{x=0}^{240} u_x $ &  $\overline{ITB}_{(1,240)}$ & Imp vs Rand. \\ \hline
    Curiosity Agent & 0.520 & \textbf{8.07} & \textbf{0.0507} &  \textbf{8.82x} \\ \hline
    Random & 0.506 & 68.7 & 0.00575 & 1.0x \\ \hline
    Orbit & \textbf{0.797} & 89.6& 0.00767 &  1.33x   \\ \hline
    Jump 7 & 0.639 & 27.0 & 0.0196 & 3.41x   \\ \hline
    Jump 10 & 0.558  & 20.0 & 0.0224 & 3.89x  \\ \hline
    Histogram 0.7 & 0.319 & 17.5 & 0.0119 & 2.07x  \\ \hline
    Histogram 0.9 & 0.505 & 48.5 & 0.00814 & 1.42x  \\ 
%     Munitions Finder & 298 & 353 & 322 & 322 \\ 
    %\hline
  \end{tabular}}
\caption{Comparison of final model performance, number of user interactions, mean incremental training benefit, and $\overline{ITB}$ relative to \textbf{random} strategy for field scenarios. We see that using a trained curiosity agent is more than 8 times more effective in utilizing user interactions than \textbf{random}, and more than 2 times more effective than the next best baseline.}
   \label{tab:simulation_results_field}
\end{table}

\vspace{-1.5em}

==> results_simulation.tex <==
% \subsection{Experiments and Results}

We evaluated our curiosity agent both in respect to average incremental training benefit (Equation~\ref{eqn:meanitb}) over the entire episode, as well as the temporal behavior of the trainee's performance during each time-step. We evaluated each strategy across 15 randomly generated environments containing between 10 to 15 obstacles. By fixing the seed at the beginning of each evaluation session, every strategy receives the same 15 environments, even though each environment is unique. For each evaluation episode, we give the agent a time budget of $T=100$, as in training. For realism, actions which do not take any time, \ie{} not moving when not training the trainee, \textit{do not count towards the time budget}.

We first measured the performance of the trainee model, as tested on all views in the exploration space, as well as the user interactions (ground truth requests), at each time-step, averaged over the 15 trial environments. These plots are shown in Figure~\ref{fig:sim_timeseries}. We can observe that the \textbf{orbit} strategy produces the highest overall trainee performance at the end of the episode---it will consistently provide 100\% coverage of the exploration space. However, since it requires the user to confirm the presence of the object at each time-step during obstruction, it also requires by far the most user interactions. The \textbf{jump} and \textbf{histogram} strategies (\ie{} subsampling) require less user interactions than orbit, and can achieve similar performance.

The curiosity agent, by intelligently deciding when to request ground truth and when to move, produced similar performance with more than 10 times fewer required user interactions as orbit, and 3-4 times less than \textbf{jump}. This corresponds to the observed qualitative behaviors of the curiosity agent---we have observed that the learned agent will continue to train on a particular view until most false positives and false negatives are removed, choosing to spend its limited time steps on particularly problematic views. Furthermore, it is less likely to request user interaction when the view is obstructed. 

\begin{figure} \centering
    \includegraphics[width=1\linewidth]{sim_timeseries}
    \caption{(top) Plot of AP vs. time step for 15 simulated scenarios. We see that the top strategies perform similarly in AP, but vary vastly in terms of number of user interactions required to get there.}
    \label{fig:sim_timeseries}
\end{figure}

We can see the benefit of this behavior more clearly by observing $\overline{ITB}$, rather than raw AP or user interactions. Using Equation~\ref{eqn:meanitb}, we computed the $\overline{ITB}_{(1,i)}$ for time steps $i=[1,100]$. This plot is shown in Figure~\ref{fig:sim_avg_itb}. 

\begin{figure} \centering
    \includegraphics[width=1\linewidth]{sim_avg_itb}
    \caption{}
    \label{fig:sim_avg_itb}
\end{figure}

We observe that when it comes to $\overline{ITB}$, the curiosity agent dominates the baseline strategies by 3.16 times the next best strategy, \textbf{jump 10}. Table~\ref{tab:simulation_results} summarizes these results quantitatively. Versus \textbf{random}, the curiosity agent produces more than 10 times $\overline{ITB}$ per user interaction. While using the curiosity agent does not necessarily produce the best performing model, \textit{it requires the least amount of user input} to get there. 

\begin{table}[h]
\resizebox{\linewidth}{!}{%
  \begin{tabular}{ c | c | c | c | c }
    \hline
    \textbf{Strategy} & $P_{100}$& $\sum_{x=0}^{100} u_x $ &  $\overline{ITB}_{(1,100)}$ & Imp. vs Rand. \\ \hline
    Curiosity Agent & 0.911 & \textbf{3.53} & \textbf{0.195} &  \textbf{10.2x} \\ \hline
    Random & 0.814 & 30.9 & 0.0191 & 1.0x \\ \hline
    Orbit & \textbf{0.943} & 41.3 & 0.0175 &  0.916x   \\ \hline
    Jump 7 & 0.850 & 12.0 & 0.0523 & 2.74x   \\ \hline
    Jump 10 & 0.778 & 9.0 & 0.0617 & 3.23x  \\ \hline
    Histogram 0.2 & 0.628 & 10.5 & 0.0388 & 2.03x  \\ \hline
    Histogram 0.7 & 0.896 & 26.6 & 0.0253 & 1.32x  \\ \hline
%     Munitions Finder & 298 & 353 & 322 & 322 \\ 
    %\hline
  \end{tabular}}
\caption{Comparison of final model performance, number of user interactions, mean incremental training benefit, and $\overline{ITB}$ relative to \textbf{random} strategy. We see that a trained curiosity agent is more than 10 times more effective in utilizing user interactions than \textbf{random}, and more than 3 times compared to the next best baseline.}
   \label{tab:simulation_results}
\end{table}

\vspace{-1.5em}
